Leveraging Redundancy in Multiple Audio Signals for Far-Field Speech Recognition

To achieve robust far-field automatic speech recognition (ASR), existing techniques typically employ an acoustic front end (AFE) cascaded with a neural transducer (NT) ASR model. The AFE output, however, could be unreliable, as the beamforming output in AFE is steered to a wrong direction. A promising way to address this issue is to exploit the microphone signals before the beamforming stage and after the acoustic echo cancellation (post-AEC) in AFE. We argue that both, post-AEC and AFE outputs, are complementary and it is possible to leverage the redundancy between these signals to compensate for potential AFE processing errors. We present two fusion networks to explore this redundancy and aggregate these multi-channel (MC) signals: (1) Frequency-LSTM based, and (2) Convolutional Neural Network based fusion networks. We augment the MC fusion networks to a conformer transducer model and train it in an end-to-end fashion. Our experimental results on commercial virtual assistant tasks demonstrate that using the AFE output and two post-AEC signals with fusion networks offers up to 25.9% word error rate (WER) relative improvement over the model using the AFE output only, at the cost of <= 2% parameter increase.

==> proposed_approaches_SLT_copy.tex <==
\section{Proposed MC fusion networks}
\label{sec:mc-fuion-net}

\begin{figure}[t]
\centering
\includegraphics[scale=0.425]{MC_UFE_SLT_fig1.pdf}
\caption{MC neural fusion transducer (MC-Fusion-Net): A NT ASR model augmented with a fusion network that exploits multiple signals.}
\label{fig:mc-fusion-net}
\end{figure}
We augment the standard NT ASR model to use multiple signals processed by different modalities. Namely, our input consists of (1) an enhanced signal produced by a traditional signal processing AFE that performs Acoustic Echo Cancellation (AEC), adaptive beamforming and noise reduction and optimal beam selection based on a signal-to-interference criterion~\cite{AudioTech} and (2) multiple raw microphone array signals after ACE (post-ACE). The multiple signals are processed by the MC fusion network (Figure~\ref{fig:mc-fusion-net}) and fused into high level representation that are input to the encoder network of the NT model. We propose two MC fusion networks. % that are described in Sections~\ref{sec:flstm} and \ref{sec:conv}.

%The standard input to a NT ASR model is a single-channel enhanced signal that has been produced by a multi-channel signal processing method. 
%The signal processing multi-channel audio front-end (AFE) we used consists of the components for Acoustic Echo Cancellation (AEC), adaptive beamforming and noise cancellation, and optimal beam selection based on a signal-to-interference criterion. The reader is referred to~\cite{AudioTech} for a complete description of the front-end. In the following, we refer to the signal that comes out of the AFE as \textit{beamformed}, or AFE output. 

%In addition to the beamformed signal, our MC Fusion Networks accept as input the raw microphone array signals after the AEC module of the aforementioned AFE. In this way, we exploit redundancies between conventionally enhanced signals and raw microphone array signals, in order to achieve better speech recognition. In the following, these signals are referred to as $raw_0, raw_1, \cdots, raw_{M-1}$ for a microphone array of $M$ sensors.  We propose two MC fusion networks that are described in Sections~\ref{sec:flstm} and \ref{sec:conv}. 

\subsection{Neural beamfomer+F-LSTM MC Fusion Network}
{\color{red} We would need to make this section smaller}


This approach utilizes a trainable neural beamformer inspired from~\cite{Wu2019} where authors used neural beamforming techniques for DNN-HMM ASR acoustic modeling. %Here, we utilize similar techniques but in the context of end-to-end ASR systems where the neural beamformer is trained jointly with the ASR system using the ASR objective function. 
%on both single and multi-channel data.
The approach is comprised of two major steps: a neural beamformer to perform spatial filtering on the multichannel inputs and a Frequency LSTM (F-LSTM)~\cite{FLSTM} layer to combine the beamformed and raw channel inputs. The architecture of the fusion network is shown in Figure~\ref{fig:bf_flstm_diagram}.
%As discussed previously, the inputs to the neural multi-channel fusion network are the raw microphone array signals after AEC and the  \textit{beamformed} from AFE. 
First, a batch normalization is applied on the frequency bins of the input signals to stabilize the training and make convergence faster.

%\subsubsection{Neural beamformer network}
\noindent \textbf{Neural beamforming network} 
The batch normalized microphone array signals, $raw_0,$ $raw_1,$  $\cdots$, $raw_{M-1}$, enter a Block Affine Transform which contains the neural beamformer network weights. 
%The batch normalized post-AEC signals $\mathbf{X}(t,omega)$ enter the neural beamforming block, 
It is a filtering operation on the input microphone array signals, and can be described as:
\begin{equation}
\label{eq:beamforming}
Y(t,\omega, \mathbf{p}) = \mathbf{w}^H(t,\omega,\mathbf{p}) \mathbf{X}(t,\omega)    
\end{equation} 
where $H$ denotes the Hermitian operation, $\mathbf{w}(t, \omega, \mathbf{p})$ is a complex weight vector for beamforming at position $\mathbf{p}$; $t$ and $\omega$ denote the time frame and angular frequency. $\mathbf{X}(t,\omega)$ is the frequency snapshot of the microphone array, given by:
\begin{equation}
\mathbf{X}(t,\omega) = \left[ raw_0(t,\omega), \cdots, raw_{M-1}(t,\omega) \right]^T    
\end{equation}

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.39]{flstm_fusion_net.pdf}
    \caption{The neural beamformer+F-LSTM MC fusion network  }
    \label{fig:bf_flstm_diagram}
\end{figure}

The complex vector  multiplication in Eq.~(\ref{eq:beamforming}) for a given frequency $\omega$ can be expressed in matrix form as:
\begin{equation}
\begin{bmatrix}
Re(Y) \\ Im(Y)
\end{bmatrix} = 
\begin{bmatrix}
Re(w_0) & Im(w_0) \\
-Im(w_0) & Re(w_0) \\
\vdots & \vdots \\
Re(w_{M-1}) & Im(w_{M-1}) \\
-Im(w_{M-1}) & Re(w_{M-1}) 
\end{bmatrix}^T
\begin{bmatrix}
Re(X_0) \\
Im(X_0) \\
\vdots \\
Re(X_{M-1}) \\
Im(X_{M-1}) 
\end{bmatrix}
\end{equation}
where  $(t, \omega, \mathbf{p})$ have been omitted for clarity and $w_i$ denotes the i-th element of the complex beamforming weight vector $\mathbf{w}$. Given this formulation, the beamforming operation can be incorporated into the neural network by using $\Omega$ $2 \times 2M$ matrices (one for each frequency bin), where $\Omega$ is the total number of frequency bins. These matrices represent the beamformer weights.
%which are initialized from the superdirective beamformer weights~\cite{himawan2010clustered,doclo2007superdirective}. 
Note that the complex signal features are treated as two real-valued inputs, so both the real and imaginary parts of the complex neural beamformer weights are learnable. 

Initially, the weights are initialized to steer the beamformer into $n_l$ look directions that are uniformly distributed around the array. During training, the $n_l$ sets of weights are optimized according to the RNN-T loss function. The neural beamformer produces $n_l$ signals in $n_l$ look directions.  
%The learned weights are used to steer the neural beamformer on a fixed set of $n_l$ look directions, which are uniformly distributed around the  array, and produces $n_l$ neural beamformed signals. %  $NB_0, NB_1, \cdots, NB_{n_l-1}$. 
 Next, all neural beamformed signals are considered together with the original microphone array signals and the AFE output. These are a total number of $n_l + M + 1$ signals. For each signal, we compute its power for each frequency bin,  by applying a square and sum operator to the real and imaginary parts. The powers then go through a ReLU activation function and a \textit{log} function (that also operate on the frequency axis), in order to get an estimate of the log power spectrum. Finally, we add another batch normalization layer operating on the frequency axis of each signal.% that we also found to help with training stability and convergence. 



\subsubsection{Signal fusion using Frequency LSTMs}
\label{sec:flstm}
Finally, the $n_l + M + 1$ signals are fused into a single hidden representation. For that, we apply an F-LSTM layer~\cite{FLSTM}. An F-LSTM is a regular LSTM layer that operates on the frequency axis instead of the time axis. 
To prepare the input for the F-LSTM, we concatenate all signals together in one vector and take chunks along the frequency axis with a certain window $w$ and stride $s$ in order to create sequences in the frequency domain of length $w$. This input is then passed through an LSTM. The output of the LSTM is projected to a hidden representation of $d_{flstm}$ that is the input to the audio encoder. 


%In the stage step, signal powers for each frequency bin are computed for each one of the neural beamformed signals $NB_i, i=1,\cdots, n_l$, as well as the original raw microphone inputs $raw_i, i=1,\cdots, M$ and the conventional superdirective beamformer output signal (\textit{beamformed}). This is done by applying a square and sum operator to the real and imaginary parts of the signal in each frequency bin. The powers then go through a \textit{relu} activation function and a \textit{log} function that also operation on the frequency bin axis, in order to get an estimate of the log power spectrum.
\subsection{Convolutional MC Fusion Network}
\label{sec:conv}

\begin{figure}[t]
\centering
\includegraphics[scale=0.35]{conv_fusion_network.pdf}
\vspace{-0.5cm}
\caption{The Convolutional MC fusion network}
\label{fig:conv-mcf}
\end{figure}

Figure \ref{fig:conv-mcf} illustrates the Convolutional Neural Network (CNN) based MC fusion network. Its design is motivated by Conv- RNN-T~\cite{radfarconvrnn} with several adaptations. First, the input channels contain the AFE output and raw microphone array signals after AEC. They are all concatenated together to form a tensor of $T \times \Omega \times C$, where $T$ is the number of time-frames, $\Omega$ is the number of frequency bins, and $C=M+1$ is the number of input channels.
%The MC inputs are first reshaped from $T\times (F\times C)$ to $T\times F\times C$ in order to apply the convolutions in the time-frequency domain. Here $T$, $F$, $C$ are the number of frames, frequency bins, and the number of channels respectively. 
The tensor is mean-normalized by the batch norm layer over the frequency axis before feeding into the two convolutional blocks. The preliminary studies show that this batch norm is critical to stablize the training. Each convolutional block has three convolutional layers and we use two blocks leading to 6 convolutional layers in total, as shown in Figure \ref{fig:conv-mcf}. Each convolutional layer is followed by a ReLU activation, and an additional residual link is added from the first ReLU input with the output. To ensure the convolution computations are causal (since our model is streamable), we zero-pad the time dimension from the left with kernel size ($K$) minus one zeros. Note that the second convolutional block downsamples the frequency bins by two ($q=2$) to maintain the model size. After the convolutional blocks, the second batch norm normalizes both the mean and scale of CNN outputs along the frequency axis, which we found to offer better convergence in our preliminary studies. 
%We use the kernel size of 5 for both time and frequency axis, i.e. $(5,5)$ and vary the stride size of the frequency axis for the first 2D CNN layer per CNN block: (from no frequency down sampling, $q=1$ to the down sampling by two, $q=2$). The second batch norm layer normalizes the CNN outputs (both mean and scale) along the frequency axis, before being fed into the dense layer.     

